Tropical Grassmannians, cluster algebras and scattering amplitudes

We provide a cluster-algebraic approach to the computation of the recently introduced generalised biadjoint scalar amplitudes related to Grassmannians ${\rm Gr}(k,n)$. A finite cluster algebra provides a natural triangulation for the tropical Grassmannian whose volume computes the scattering amplitudes. Using this method one can construct the entire colour-ordered amplitude via mutations starting from a single term.

==> figures/dual26.tex <==

\begin{tikzpicture}[scale=0.75]

  \begin{scope}[canvas is plane={O(0,0,0)x(0,1,0)y({cos(240)},0,{sin(240)})}]
      \draw[fill=green, opacity=0.2, line width=1] (4,0) arc (0:180:4);
      \draw[opacity=1, line width=1] (45:4) arc (45:135:4);
   \end{scope}
  
   \begin{scope}[canvas is plane={O(0,0,0)x(0,1,0)y({cos(120)},0,{sin(120)})}]
     \draw[fill=red, opacity=0.2, line width=1] (4,0) arc (0:180:4);
     \draw[opacity=1, line width=1] (45:4) arc (45:135:4);

   \end{scope}

   \draw[red] (0,0,0) -- (0,1,0);
   \draw[blue] (0,0,0) -- (0,0,1);
   \draw[green] (0,0,0) -- (1,0,0);


   \begin{scope}[canvas is plane={O(0,0,0)x(0,1,0)y({cos(0)},0,{sin(0)})}]
     \draw[fill=blue, opacity=0.2, line width=1] (4,0) arc (0:180:4);
     \draw[opacity=1, line width=1] (45:4) arc (45:135:4);
   \end{scope}
        
   % \begin{scope}[canvas is plane={O(0,0,0)x({-sin(45)}, {cos(45)}, 0)y(0,0,1)}]
   %   % \draw[fill=gray, opacity=1, line width=1] (0:4) arc (0:-60:4) -- (0,0);
   %   \draw (0,0) -- (4,0);

   % \end{scope}


   \pgfmathsetmacro{\ang}{0}
 %   \draw[green] (0,0,0) -- ({4*cos(120)*cos(\ang)},4*sin(\ang),{4*sin(120)*cos(\ang)});


   \begin{scope}[canvas is plane={O(0,0,0)x(1,0,0)y(0,0,1)}]
     \draw (0,0) circle (4);
   \end{scope}

   
\end{tikzpicture}

  	


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../tropical"
%%% End:

